Maximizing Stochastic Monotone Submodular Functions

We study the problem of maximizing a stochastic monotone submodular function with respect to a matroid constraint. Due to the presence of diminishing marginal values in real-world problems, our model can capture the effect of stochasticity in a wide range of applications. We show that the adaptivity gap -- the ratio between the values of optimal adaptive and optimal non-adaptive policies -- is bounded and is equal to e/(e-1). We propose a polynomial-time non-adaptive policy that achieves this bound. We also present an adaptive myopic policy that obtains at least half of the optimal value. Furthermore, when the matroid is uniform, the myopic policy achieves the optimal approximation ratio of 1-1/e.

==> extensions.tex <==
\section{\upt{Extensions and Discussions}} \label{sec:extensions}

%\upt{
%\subsection{Choosing Elements With Replacement} \label{sec:mult}
%So far, we have assumed that there is no benefit in selecting an element multiple times since once an element is picked by a policy, its realized value does not changed. However, this assumption is made only to simplify the presentation and has no effect on our results. This follows from the observation that one can create identical and independent copies of each random variable in order to simulate multiplicity. 
%Hence, all our approximation guarantees and the adaptivity gap, which are {\em independent} of the size of the problem, will hold when multiple selection of an element might change its value.
%\footnote{\upt{Our tightness results for approximation guarantees come from deterministic examples, they still hold when the multiplicity is allowed.}} \\
%%
%%For , with the same reasoning (by creating independent copies) we conclude that our upper bound holds even when the multiplicity is allowed, i.e., the expected value of no adaptive policy is strictly better than $\tfrac{e}{e-1}$ times the expected value of the best non-adaptive policy. \\
%%For the lower bound, in Section~\ref{sec:tightexample} we show how to make a tight example with the same lower bound for the cases in which multiplicity is allowed.
%%
%%Hence, all the results in our paper still hold if in our model we allow multiple selections of the elements. \\
%This is in contrast with covering and threshold problems in which the goal is to reach a value of function above a certain hard-constrained threshold. For instance, in the problem of stochastic set cover problem (where the goal is to cover \emph{all} the elements of a ground set using the minimum number of a given collection of its subsets), allowing to choose multiple copies of an element significantly reduces the adaptivity gap as shown in~\cite{GoemansV06}.
%}


%\begin{remark}
%A tight example for the model in which multiplicity is allowed follows immediately from the above instance. Consider a ground set $N = \{1, 2, \cdots, n\}$ and a
%collection $\F = \{X^{(i)} = \{i\}|1 \leq i \leq n\}$. Any non-adaptive policy can be described by an $n$-tuple $(k_1, k_2, \cdots, k_n)$ where $k_i$ is the number of times $X^{(i)}$ is included in the set picked by the policy. The proof of Lemma~\ref{lem:example_nonadaptive} directly applies and an upper bound for its value is immediately established. Moreover, a similar adaptive policy $\P$ can be defined as follows: start with $i = 1$ and pick the $i$-th element until its corresponding subset is realized as $\{i\}$. Then increase $i$ by one. Continue the iteration until $i = n+1$ or the number of actions reaches $n^2$. Lemma~\ref{lem:example_adaptive} with the  same proof immediately follows. This shows the same lower bound of adaptivity gap for the problem.
%\end{remark}

%\upt{
%\subsection{Unbounded Adaptivity Gap Without the Independence Assumption} \label{apx:unbouned}
%In this section, we present an example that shows that the adaptivity gap in general can be at least $n/2$. \\
%Consider an instance of SMSM with the ground set $\A = \{X_0, X_1, \cdots, X_n\}$, where $X_0$, with equal probability of ${1\over n}$,  takes one of the values in $\{1,2,\ldots,n\}$. Also, for $i$, $1\le i\le n$, we have $X_i = M \times \textbf{I}\{x_0 = i\}$ for some $M \gg n$, i.e., $x_j = M$ if $x_0 = j$; otherwise, $x_j=0$.
%%
%The goal is to maximize a \emph{linear} function $f$ that correspond to the sum of the realized values of the chosen elements.
%% $f(X_0, X_1, \cdots, X_n) = X_0 + X_1 + \cdots + X_n$.
%The constraint is to select at most two elements, i.e., a basis from the matroid $\M = (\A, \{S \subseteq \A, |S| \leq 2\})$.
%}\upt{
%It is easy to see that any non-adaptive algorithm would yield a value of at most $2M/n$. However, an adaptive policy that selects $X_0$ first, and then selects $j=x_0$ and obtains a value of at least $M$ (or $M+j$ to be more precise). Hence, the adaptivity gap is at least $n/2$.
%}


%\subsection{\upt{Computationing $F$}} \label{sec:f_computation}
%%
%\upt{
%The problem of calculating function $F$ and functions similar to it has appeared in many of the related works and is usually solved via sampling. For instance, in the framework of~\cite{VondrakThesis07, Vondrak08}, 
%where they deal with a similar notion of $F$, but only with Bernoulli distribution for all distributions $g_i$-s, they show that with repeated sampling one can get an estimation of $F$ within a multiplicative error of $1\pm 1/\textrm{poly}(n)$. The following proposition provides a generalization of their result to the Lipschitz continuous functions.
%\begin{proposition}
%\label{lem:sampling}
%Suppose $f$ is $K$-Lipschitz continuos and for all $i$, $\Var[X_i] \leq \V$. Then, the average value of $\Phi(\Theta_S)$ for $t = \lceil K^2 n^5 \V \rceil$ independent samples is within the interval $(\E[\Phi(\Theta_S)] - n^{-2}, (\E[\Phi(\Theta_S)] + n^{-2})$ with probability $1-n^{-2}$.
%\end{proposition}
%\begin{proof}{Proof:}
%Note that $F(S) = \E[\Phi(\Theta_S)]$. By Lemma~\ref{lem:lipbound} in Appendix~\ref{sec:lipbound} we know that $\Var[\Phi(\Theta_S)] \leq K^2 |S|^2 \V$. Suppose that we take $t$ independent samples of the value of $\Phi(\Theta_S)$ and take their average as an estimation for the actual value of $\Phi(\Theta_S)$. The derived sample will have a variance lower than $K^2 |S|^2 \V/t$. The proof is completed by taking $t = \lceil K^2 n^5 \V \rceil$ and applying Chebyshev inequality.
%% \footnote{
%% \textcolor{red}{
%Note that if we have an upperbound for the values of $f$ (for instance, as in the problem of~\cite{VondrakThesis07, Vondrak08} where $X$'s can only take 0/1 values) then we can use Chernoff inequality in the proof. That allows us to get the same bounds by only $O(\log K + \log n + \log \V)$ samples. Also, since in this case the values $F$ can take would be finite, one can interpret these bounds via multiplicative error terms.
%%}}
%\qed\end{proof}
%}

%****************************************************************

%\upt{
%\subsection{Intersection of $\kappa$ Matroids} \label{sec:intersection}
%If the feasible domain of the problem is the intersection of $\kappa$ matroids $\M_1 = (\A_1, \I_1), \M_2=(\A_2, \I_2), \cdots, \M_{\kappa}=(\A_{\kappa}, \I_{\kappa})$, then the approximation ratio of our myopic algorithm will be $\tfrac{1}{1+\kappa}$. To show that, we first note that in order to derive all inequalities in the proof of Theorem~\ref{halfapprox} up to Eq.~\ref{eq:kmatroid} we only used the  facts that {\em i}) $F$ is a monotone submodular function, and {\em ii})
%At each step, our policy picks the feasible element with the highest marginal value. In other words, those inequalities do not rely on the fact that the feasible domain is a single matroid. Now, we can use the generalization of Lemma~\ref{lem:fnwp1} to $\kappa$ matroids. The following is a property of the intersection of $\kappa$ matroids and is proved in~\cite{FisherNW78-2}. Again, let $k$ be the number of steps our myopic policy take and let $S = S_k$ denote the final selection of this policy.
%%
%\begin{lemma}~\cite{FisherNW78-2}\label{lem:fnwp2}
%Let $P \in \I_1\cap \I_2 \cup \cdots \cup \I_{\kappa}$ be any arbitrary subset in the intersection of $\kappa$ matroids, $\M_1, \M_2, \cdots, \M_{\kappa}$. For $1 \leq i \leq k$ let $C_{i} = P \cap (U_{i+1} \setminus U_{i})$. Then, for every $1 \leq t \leq k$ we have $\sum_{i=1}^{t} |C_i| \leq \kappa t$.
%\end{lemma}
%%
%Now, using the above lemma Eq.~\ref{eq:kmatroid} can be rewritten as below.
%\begin{eqnarray*}
%\E[F(P)] - \E[F(S)] & \leq & \sum_{j = 1}^{k}
%\int_{s_{j-1}: S_{j - 1}\in \I} \left(\E[\sum_{t=1}^{j} |C_t||s_{j-1}] \E[\Delta_j - \Delta_{j + 1}|s_{j-1}]\right) \Pr[s_{j-1}] ds_{j-1}\\
%%
%&\leq& \sum_{j = 1}^{k}
%\int_{s_{j-1}: S_{j - 1}\in \I} \kappa j \E[(\Delta_j - \Delta_{j + 1})|s_{j-1}] \Pr[s_{j-1}] ds_{j-1} \\
%%
% & = & \sum_{j = 1}^{k}
%\int_{s_{j-1}: S_{j - 1}\in \I}  \kappa\E[\Delta_j|s_{j-1}] \Pr[s_{j-1}] ds_{j-1} \\
%%
% & = & \kappa\sum_{j = 1}^{k}  \E[\Delta_j] \\
%%
% & = & \kappa\E[F(S)].
%\end{eqnarray*}
%This shows $\E[F(P)] \le (\kappa+1) \E[F(S)]$, which results in the myopic policy being a $\tfrac{1}{\kappa+1}$-approximation of the optimal adaptive policy.
%}
%
%See \cite{GolovinK11_2} for a similar result.
